A Matrix Product State Model for Simultaneous Classification and Generation

Quantum machine learning (QML) is a rapidly expanding field that merges the principles of quantum computing with the techniques of machine learning. One of the powerful mathematical frameworks in this domain is tensor networks. These networks are used to approximate high-order tensors by contracting tensors with lower ranks. Initially developed for simulating quantum systems, tensor networks have become integral to quantum computing and, by extension, to QML. Drawing inspiration from these quantum methods, specifically the Matrix Product States (MPS), we apply them in a classical machine learning setting. Their ability to efficiently represent and manipulate complex, high-dimensional data makes them effective in a supervised learning framework. Here, we present an MPS model, in which the MPS functions as both a classifier and a generator. The dual functionality of this novel MPS model permits a strategy that enhances the traditional training of supervised MPS models. This framework is inspired by generative adversarial networks and is geared towards generating more realistic samples by reducing outliers. In addition, our contributions offer insights into the mechanics of tensor network methods for generation tasks. Specifically, we discuss alternative embedding functions and a new sampling method from non-normalized MPSs.

==> images/biblio.tex <==
\begin{thebibliography}{20}


\bibitem{peps:supervised}
Cheng, Song, Lei Wang, and Pan Zhang. "Supervised learning with projected entangled pair states." Physical Review B 103.12 (2021): 125117.

\bibitem{unitary_tn:sampling}
Ferris, Andrew J., and Guifre Vidal. "Perfect sampling with unitary tensor networks." Physical Review B 85.16 (2012): 165146.

\bibitem{mps:supervised}
E. Miles, Schwab. "Supervised Learning with Quantum-Inspired Tensor Networks." Advances in Neural Information Processing Systems 29, 4799 (2016)

\bibitem{mps:unsupervised}
Han, Zhao-Yu, et al. "Unsupervised generative modeling using matrix product states." Physical Review X 8.3 (2018): 031012.

\bibitem{mps:2dsystems}
Bruognolo, Benedikt, et al. "Matrix product state techniques for two-dimensional systems at finite temperature." arXiv preprint arXiv:1705.05578 (2017).

\bibitem{DMRG}
Schollwöck, Ulrich. "The density-matrix renormalization group in the age of matrix product states." Annals of Physics 326.1 (2011): 96-192.


\bibitem{peps:generative}
Vieijra, Tom, Laurens Vanderstraeten, and Frank Verstraete. "Generative modeling with projected entangled-pair states." arXiv preprint arXiv:2202.08177 (2022).

\bibitem{mps:samples}Liu, Jing, et al. "Tensor networks for unsupervised machine learning." Physical Review E 107.1 (2023): L012103.

\bibitem{lps}Glasser, Ivan, et al. "Expressive power of tensor-network factorizations for probabilistic modeling." Advances in neural information processing systems 32 (2019).

\bibitem{mps:positive_unlabeled_learning}Žunkovič, Bojan. "Positive unlabeled learning with tensor networks." Neurocomputing (2023): 126556.


\bibitem{mps:privacy_preserving}Pozas-Kerstjens, Alejandro. "Privacy-preserving machine learning with tensor networks." Bulletin of the American Physical Society (2023).

\bibitem{torch:autograd}
Paszke, Adam, et al. "Automatic differentiation in pytorch." (2017).

\bibitem{pytorch}Paszke, Adam, et al. "Pytorch: An imperative style, high-performance deep learning library." Advances in neural information processing systems 32 (2019).

\bibitem{mps:discrete}Bonnevie, Rasmus, and Mikkel N. Schmidt. "Matrix product states for inference in discrete probabilistic models." The Journal of Machine Learning Research 22.1 (2021): 8396-8443.

\bibitem{rectflow}Caterini, Anthony L., et al. "Rectangular flows for manifold learning." Advances in Neural Information Processing Systems 34 (2021): 30228-30241.

\bibitem{gan}Goodfellow, Ian, et al. "Generative adversarial nets." Advances in neural information processing systems 27 (2014).


% \bibitem{KLdiv:1}Goodfellow, Ian, Yoshua Bengio, and Aaron Courville. Deep learning. MIT press, 2016.

% \bibitem{KLdiv:2}LeCun, Yann, Yoshua Bengio, and Geoffrey Hinton. "Deep learning." nature 521.7553 (2015): 436-444.




\bibitem{mpspeps:intro}R. Orús, A Practical Introduction to Tensor Networks: Matrix Product States and Projected Entangled Pair States, Ann. Phys. 349, 117 (2014).



\bibitem{mps:approximations}Dalzell, Alexander M., and Fernando GSL Brandão. "Locally accurate MPS approximations for ground states of one-dimensional gapped local Hamiltonians." Quantum 3 (2019): 187.
% \bibitem{}
\bibitem{DMRG2} White, Steven R. "Density matrix formulation for quantum renormalization groups." Physical review letters 69.19 (1992): 2863.%

\bibitem{DMRG3}White, Steven R. "Density-matrix algorithms for quantum renormalization groups." Physical review b 48.14 (1993): 10345.%

\bibitem{tn:nutshell}Biamonte, Jacob, and Ville Bergholm. "Tensor networks in a nutshell." arXiv preprint arXiv:1708.00006 (2017).


\bibitem{sweeping}Chan, Garnet Kin, et al. "Matrix product operators, matrix product states, and ab initio density matrix renormalization group algorithms." The Journal of chemical physics 145.1 (2016).

\bibitem{gradient_descent} Ruder, Sebastian. "An overview of gradient descent optimization algorithms." arXiv preprint arXiv:1609.04747 (2016).

\bibitem{adam}Kingma, Diederik P., and Jimmy Ba. "Adam: A method for stochastic optimization." arXiv preprint arXiv:1412.6980 (2014).

\bibitem{mps:introduced} Fannes, Mark, Bruno Nachtergaele, and Reinhard F. Werner. "Finitely correlated states on quantum spin chains." Communications in mathematical physics 144 (1992): 443-490.

\bibitem{mps:data_compression}Bengua, Johann A., et al. "Matrix product state for higher-order tensor compression and classification." IEEE Transactions on Signal Processing 65.15 (2017): 4019-4030.


\bibitem{tn:intro}Orús, Román. "Tensor networks for complex quantum systems." Nature Reviews Physics 1.9 (2019): 538-550.


\bibitem{mera}Vidal, Guifre. "Entanglement renormalization." Physical review letters 99.22 (2007): 220405.

\bibitem{ttn} Cheng, Song, et al. "Tree tensor networks for generative modeling." Physical Review B 99.15 (2019): 155131.


\bibitem{mps:tt_decomp}Oseledets, Ivan V. "Tensor-train decomposition." SIAM Journal on Scientific Computing 33.5 (2011): 2295-2317.

\bibitem{tn:np-complete}Håstad, Johan. "Tensor rank is NP-complete." Automata, Languages and Programming: 16th International Colloquium Stresa, Italy, July 11–15, 1989 Proceedings 16. Springer Berlin Heidelberg, 1989.

\bibitem{tn:ill-posed}De Silva, Vin, and Lek-Heng Lim. "Tensor rank and the ill-posedness of the best low-rank approximation problem." SIAM Journal on Matrix Analysis and Applications 30.3 (2008): 1084-1127.

\bibitem{penrose}Penrose, Roger. "Applications of negative dimensional tensors." Combinatorial mathematics and its applications 1 (1971): 221-244.


\bibitem{mps:quantum1}Perez-Garcia, David, et al. "Matrix product state representations." arXiv preprint quant-ph/0608197 (2006).

\bibitem{mps:quantum2}Verstraete, Frank, and J. Ignacio Cirac. "Matrix product states represent ground states faithfully." Physical review b 73.9 (2006): 094423.

\bibitem{mps:quantum3}Hastings, Matthew B. "An area law for one-dimensional quantum systems." Journal of statistical mechanics: theory and experiment 2007.08 (2007): P08024.


\bibitem{mps:easier_training}Efthymiou, Stavros, Jack Hidary, and Stefan Leichenauer. "Tensornetwork for machine learning." arXiv preprint arXiv:1906.06329 (2019).


\bibitem{mps:unbiased_mcmc}Ferris, Andrew J. "Unbiased Monte Carlo for the age of tensor networks." arXiv preprint arXiv:1507.00767 (2015).


\bibitem{mnist}Christopher J.C. Burges Yann LeCun, Corinna Cortes, “MNIST handwritten digit database,” \url{http://yann.lecun.com/exdb/mnist/}.

\bibitem{fmnist}Xiao, Han, Kashif Rasul, and Roland Vollgraf. "Fashion-mnist: a novel image dataset for benchmarking machine learning algorithms." arXiv preprint arXiv:1708.07747 (2017).

\bibitem{mps:curseofdim}Bridgeman, Jacob C., and Christopher T. Chubb. "Hand-waving and interpretive dance: an introductory course on tensor networks." Journal of physics A: Mathematical and theoretical 50.22 (2017): 223001.

\bibitem{flouris2025}
Flouris, Kyriakos, Anna Volokitin, Gustav Bredell, and Ender Konukoglu. "Explicit and data-efficient encoding via gradient flow." arXiv preprint arXiv:2412.00864 (2025).

\bibitem{PhysRevB.105.235122}
Flouris, Kyriakos, Miller Mendoza Jimenez, and Hans J. Herrmann. "Curvature-induced quantum spin-Hall effect on a Möbius strip." *Physical Review B* 105.23 (2022): 235122.


\bibitem{canonicalform}
Matrix Product States: Canonical Forms, \url{https://muellergroup.lassp.cornell.edu/bt2020chap4.pdf}, (accessed on 24.10.2023).



\end{thebibliography}%

